The Pitfalls and Promise of Conformal Inference Under Adversarial Attacks

In safety-critical applications such as medical imaging and autonomous driving, where decisions have profound implications for patient health and road safety, it is imperative to maintain both high adversarial robustness to protect against potential adversarial attacks and reliable uncertainty quantification in decision-making. With extensive research focused on enhancing adversarial robustness through various forms of adversarial training (AT), a notable knowledge gap remains concerning the uncertainty inherent in adversarially trained models. To address this gap, this study investigates the uncertainty of deep learning models by examining the performance of conformal prediction (CP) in the context of standard adversarial attacks within the adversarial defense community. It is first unveiled that existing CP methods do not produce informative prediction sets under the commonly used $l_{\infty}$-norm bounded attack if the model is not adversarially trained, which underpins the importance of adversarial training for CP. Our paper next demonstrates that the prediction set size (PSS) of CP using adversarially trained models with AT variants is often worse than using standard AT, inspiring us to research into CP-efficient AT for improved PSS. We propose to optimize a Beta-weighting loss with an entropy minimization regularizer during AT to improve CP-efficiency, where the Beta-weighting loss is shown to be an upper bound of PSS at the population level by our theoretical analysis. Moreover, our empirical study on four image classification datasets across three popular AT baselines validates the effectiveness of the proposed Uncertainty-Reducing AT (AT-UR).

==> Supplemental_v1.tex <==
\clearpage
\appendix

\thispagestyle{empty}
% dates when survey collected, version
% sample responses

%
% For one-column format, uncomment the following:
\onecolumn 
\section{Adaptive Prediction Sets \citep{romano2020classification}}
\label{app_sec:aps}
We introduce one example of prediction set function, i.e., APS conformal prediction used in our experiment. Assume we have the prediction distribution $\pi(x)=f_{\theta}(x)$ and order this probability vector with the descending order $\pi_{(1)}(x) \ge \pi_{(2)}(x) \geq \ldots \geq \pi_{(K)}(x)$. We first define the following generalized conditional quantile function,
\begin{align} \label{eqn:gcq}
  Q(x; \pi, \tau) & = \min \{ k \in \{1,\ldots,K\} \ : \ \pi_{(1)}(x) + \pi_{(2)}(x) + \ldots + \pi_{(k)}(x) \geq \tau \},
\end{align}
which returns the class index with the generalized quantile $\tau\in[0,1]$. The function $\gS$ can be defined as
\begin{align} \label{eqn:S}
    \mathcal{S}(x, u ; \pi, \tau) & = 
    \begin{cases}
    \text{ `$y$' indices of the $Q(x ; \pi,\tau)-1$ largest $\pi_{y}(x)$},
    & \text{ if } u \leq V(x ; \pi,\tau) , \\
    \text{ `$y$' indices of the $Q(x ; \pi,\tau)$ largest $\pi_{y}(x)$},
    & \text{ otherwise},
    \end{cases}
\end{align}
where
\begin{align*}
    V(x; \pi, \tau) & =  \frac{1}{\pi_{(Q(x ; \pi, \tau))}(x)} \left[\sum_{k=1}^{Q(x ; \pi, \tau)} \pi_{(k)}(x) - \tau \right].
\end{align*}
It has input $x$, $u \in [0,1]$, $\pi$, and $\tau$ and can be seen as a generalized inverse of Equation~\ref{eqn:gcq}. 

On the calibration set, we compute a generalized inverse quantile conformity score with the following function,
\begin{align}
    E(x,y,u;\pi) & = \min \left\{ \tau \in [0,1] : y \in \gS(x, u ; \pi, \tau) \right\},
\end{align}
which is the smallest quantile to ensure that the ground-truth class is contained in the prediction set $\gS(x, u ; \pi, \tau)$. With the conformity scores on calibration set $\{E_i\}_{i=1}^{n_c}$, we compute the $\ceil{(1-\alpha)(1+n_c)}$th largest value in the score set as $\hat\tau_{\text{cal}}$. During inference, the prediction set is generated with $\gS(x^*, u ; \pi^*, \hat\tau_{\text{cal}})$ for a novel test sample $x^*$.




\section{More Experimental Details}
\label{app_sec:exp_details}
\paragraph{APS Setting.} We use the default setting of APS specified in the official code of \cite{angelopoulos2020uncertainty}, i.e., first use temperature scaling \citep{platt1999probabilistic,guo2017calibration} to calibrate the prediction distribution then compute the generalized inverse quantile conformity score to perform the calibration and conformal prediction. 
\paragraph{Hyperparameter and Baseline Setting.} As mentioned in the main paper, we use $a=1.1$ and search $b$ from the discrete set $\{2.0,3.0,4.0,5.0\}$ in Beta distribution since the parameter combinations perform well in our pilot study and satisfy the goal of focusing on promising samples. The learning rate and weight decay of AT, FAT and TRADES are determined by grid search from \{1e-4,3e-4,1e-3,3e-3,1e-2\} and \{1e-3,1e-4,1e-5\} respectively. We compute the class weight for FAT using the output of a softmax function with error rate of each class as input. The temperature in the softmax function is set as 1.0. For TRADES, we follow the default setting $\beta=6.0$ for the KL divergence term \citep{zhang2019theoretically}. Our AT-UR method also determines the learning rate and weight decay using the grid search with the same mentioned grid. For TRADES, we weight both the cross-entropy loss and KL divergence loss with the Beta density function based on TCPR. 

\paragraph{CP Curve.} The CP curve in Fig.~\ref{fig:cp_curve} is obtained by using different threshold values, for instance, using the linspace function in numpy \citep{harris2020array} with \code{np.linspace(0.9,1.1,200)}$\times\hat\tau_{\text{cal}}$ generates 200 different (coverage, PSS) points. 

\section{More Experimental Results}
\label{app_sec:exp_results}
Note that this paper uses CP as the inference method to achieve a coverage guarantee, which is orthogonal to the Top-1 inference method. Thus, Top-1 accuracy is not a relevant metric in the context of CP inference. Nevertheless, we show the Top-1 accuracy of tested methods in Tab.~\ref{tab:top_1_acc}. Using AT-UR generally worsens the Top-1 accuracy, especially for TRADES. However, note that using TRADES-Beta-EM can improve the Top-1 robust accuracy of TRADES-Beta on CIFAR10 and TRADES-EM on Caltech256. This result again confirms the observation that Top-1 accuracy is not necessarily correlated with CP-efficiency. \revise{We use the AutoAttack (AA) \cite{croce2020reliable} to evaluate our method with AT, as AA is the most popular adversarial attack in literature due to its effectiveness. See Tab.~\ref{tab:autoattack} for the result. Under AA, the performance of our approach is also substantially better than the AT baseline. Interestingly, the robust accuracy under AA drops while the prediction set size reduced (CP efficiency is improved). }

\begin{figure}[t]
     \centering
     \includegraphics[width=\textwidth]{Figure/sec_7_FAT_cp_curve_all_data.pdf}
    \caption{The CP curve of coverage versus prediction set size using FAT.}
    \label{fig:cp_curve_fat}
\end{figure}

\begin{figure}[t]
     \centering
     \includegraphics[width=\textwidth]{Figure/sec_7_TRADES_cp_curve_all_data.pdf}
    \caption{The CP curve of coverage versus prediction set size using TRADES.}
    \label{fig:cp_curve_trades}
\end{figure}


Fig.~\ref{fig:cp_curve_fat} and Fig.~\ref{fig:cp_curve_trades} shows the CP curve of FAT and TRADES when they are combined with EM and Beta on three datasets. It demonstrates that the CP-efficiency is also improved when using FAT and TRADES as in the experiment using AT. In most cases (5 out of 6), AT-UR (either EM or Beta) has a lower PSS than the corresponding baseline within a large range of coverage. 


\begin{table}[t]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{|c|cc|cc|cc|cc|}
\hline
     Dataset   & \multicolumn{2}{c|}{CIFAR10}     & \multicolumn{2}{c|}{CIFAR100}    & \multicolumn{2}{c|}{Caltech256}  & \multicolumn{2}{c|}{CUB200}      \\ \hline 
     Metric   & \multicolumn{1}{c|}{Cvg} & NPSS & \multicolumn{1}{c|}{Cvg} & NPSS & \multicolumn{1}{c|}{Cvg} & NPSS & \multicolumn{1}{c|}{Cvg} & NPSS \\ \hline
AT      & \multicolumn{1}{c|}{90.55(0.51)}     &   31.0(0.7)   & \multicolumn{1}{c|}{90.45(0.59) }     &  23.79(0.80)    & \multicolumn{1}{c|}{91.35(0.85)}     &   16.8(0.8)   & \multicolumn{1}{c|}{90.33(0.89) }     &   18.7(1.1)   \\ %\hline
AT-EM$^*$   & \multicolumn{1}{c|}{90.39(0.48) }     &  \textbf{30.5(0.5)}    & \multicolumn{1}{c|}{90.35(0.82) }     & \textbf{22.05(1.02)}     & \multicolumn{1}{c|}{91.09(0.79) }     &  16.1(1.0)    & \multicolumn{1}{c|}{90.08(1.10) }     &   17.4(1.3)   \\ %\hline
AT-Beta$^*$ & \multicolumn{1}{c|}{90.46(0.51) }     &   31.1(0.7)   & \multicolumn{1}{c|}{90.10(0.51)  }     &  22.64(0.65)    & \multicolumn{1}{c|}{90.20(0.84) }     &   \textbf{13.8(1.0)}   & \multicolumn{1}{c|}{90.17 (1.06)}     &   17.6(1.1)   \\ %\hline
AT-Beta-EM$^*$   & \multicolumn{1}{c|}{90.65(0.62) }     &  31.0(0.8)    & \multicolumn{1}{c|}{90.40(0.60)}     & 22.53(0.91)     & \multicolumn{1}{c|}{90.81(1.00)}     &   14.1(1.4)   & \multicolumn{1}{c|}{90.31(0.84) }     &  \textbf{16.5(0.9)}    \\ \hline
FAT   & \multicolumn{1}{c|}{90.69(0.61)}     &   31.6(0.7)  & \multicolumn{1}{c|}{90.41(0.67) }     & 23.54(0.81)     & \multicolumn{1}{c|}{90.70(0.77)}     & 16.2(0.9)      & \multicolumn{1}{c|}{ 90.50(1.17)}     &  19.7(1.4)    \\
FAT-EM$^*$  & \multicolumn{1}{c|}{ 90.54(0.68) }     &   30.6(0.6)  & \multicolumn{1}{c|}{90.00(0.82)}     & 23.47(2.71)     & \multicolumn{1}{c|}{ 90.55(0.79) }     & 15.5(1.0)     & \multicolumn{1}{c|}{89.89(0.919) }     &  17.8(1.0)     \\
FAT-Beta$^*$   & \multicolumn{1}{c|}{90.47(0.51)}     &   31.6(0.8)   & \multicolumn{1}{c|}{90.22(0.47)}     &  23.15(0.71)     & \multicolumn{1}{c|}{89.90(0.70)}     &  13.5(0.9)    & \multicolumn{1}{c|}{ 89.92(0.84) }     &  17.7(0.9)     \\
FAT-Beta-EM$^*$   & \multicolumn{1}{c|}{90.71(0.61)}     &  \textbf{30.4(0.7)}   & \multicolumn{1}{c|}{90.36(0.50) }     & \textbf{22.28(0.63)}     & \multicolumn{1}{c|}{90.41(0.61) }     &   \textbf{13.1(1.1)}    & \multicolumn{1}{c|}{ 89.88(0.91) }     &  \textbf{17.2(0.8)}    \\
\hline
TRADES   & \multicolumn{1}{c|}{90.72(0.62) }     & 33.1(0.9)     & \multicolumn{1}{c|}{90.35(0.57) }     &  27.60(0.97)    & \multicolumn{1}{c|}{90.82(0.81) }     &  17.4(1.3)    & \multicolumn{1}{c|}{ 90.38(0.76) }     &  26.1(1.3)     \\ 
TRADES-EM$^*$   & \multicolumn{1}{c|}{90.54(0.40) }     &  \textbf{31.6(0.5)}   & \multicolumn{1}{c|}{90.36(0.71) }     & \textbf{26.76(1.00)}     & \multicolumn{1}{c|}{ 90.68(0.87) }     & \textbf{15.1(1.5)}     & \multicolumn{1}{c|}{ 90.05(0.76)}     & \textbf{22.5(1.4)}      \\
TRADES-Beta$^*$  & \multicolumn{1}{c|}{90.41(0.56) }     &   33.0(0.9)  & \multicolumn{1}{c|}{90.14(0.85)}     &  27.22(1.42)    & \multicolumn{1}{c|}{90.48(0.70) }     &  15.1(1.1)    & \multicolumn{1}{c|}{89.83(0.84) }     &  24.8(1.3)    \\
TRADES-Beta-EM$^*$   & \multicolumn{1}{c|}{90.01(0.40)}     &  32.1(0.6)   & \multicolumn{1}{c|}{90.54(0.24)}     &   26.55(0.35)   & \multicolumn{1}{c|}{90.52(0.74) }     &  15.5(1.2)    & \multicolumn{1}{c|}{90.16(1.12)}     & 24.3(1.3) \\
\hline
\end{tabular}
}
\vspace{-0.3cm}
\caption{\revise{Comparison of AT baselines and the proposed AT-UR variants denoted with $^*$. The average coverage (Cvg) and prediction set size normalized by the class number (NPSS, \%) are presented. } }
\vspace{-0.5cm}
\label{tab:main_normalized}
\end{table}




\begin{table}[t]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{|c|cc|cc|cc|cc|}
\hline
     Dataset   & \multicolumn{2}{c|}{CIFAR10}     & \multicolumn{2}{c|}{CIFAR100}    & \multicolumn{2}{c|}{Caltech256}  & \multicolumn{2}{c|}{CUB200}      \\ \hline 
     Metric   & \multicolumn{1}{c|}{Std. Acc.} & Rob. Acc. & \multicolumn{1}{c|}{Std. Acc.} & Rob. Acc. & \multicolumn{1}{c|}{Std. Acc.} & Rob. Acc. & \multicolumn{1}{c|}{Std. Acc.} & Rob. Acc. \\ \hline
AT      & \multicolumn{1}{c|}{ 89.76(0.15)  }     &  50.17(0.91)    & \multicolumn{1}{c|}{68.92(0.38) }     &  28.49(1.14)    & \multicolumn{1}{c|}{ 75.28(0.51) }     &  47.53(0.67)  & \multicolumn{1}{c|}{65.36(0.27) }     &  26.29(0.45)   \\ %\hline
AT-EM$^*$   & \multicolumn{1}{c|}{ 90.02(0.10) }     &  48.92(0.39)   & \multicolumn{1}{c|}{68.39(0.51) }     &  28.33(0.73)     & \multicolumn{1}{c|}{74.62(0.22)   }     &  46.23(0.44)   & \multicolumn{1}{c|}{ 64.75(0.33) }     &    25.60(0.25)  \\ %\hline
AT-Beta$^*$ & \multicolumn{1}{c|}{ 89.81(0.22)}     &   47.50(0.78)  & \multicolumn{1}{c|}{68.50(0.28) }     &  28.04(0.57)   & \multicolumn{1}{c|}{ 74.66(0.54)  }     &   45.40(0.59)  & \multicolumn{1}{c|}{ 64.62(0.17)  }     &  25.57(0.41)   \\ %\hline
AT-Beta-EM$^*$   & \multicolumn{1}{c|}{ 90.00(0.06)}     &  46.69(0.71)   & \multicolumn{1}{c|}{ 68.45(0.35)}     &    27.20(1.08)   & \multicolumn{1}{c|}{74.71(0.36)}     &  44.88(0.60)     & \multicolumn{1}{c|}{ 64.44(0.22) }     &  25.32(0.38) \\ \hline
FAT      & \multicolumn{1}{c|}{ 89.96(0.25)}     &   49.12(0.70)   & \multicolumn{1}{c|}{68.80(0.38)}     &    28.97(0.53)   & \multicolumn{1}{c|}{75.20(0.33) }     &  47.09(0.70)  & \multicolumn{1}{c|}{ 65.01(0.19) }     &  25.21(0.57)   \\ %\hline
FAT-EM$^*$   & \multicolumn{1}{c|}{ 90.19(0.07)}     &  48.31(0.80)    & \multicolumn{1}{c|}{68.76(0.39)  }     & 25.84(3.54)   & \multicolumn{1}{c|}{74.59(0.20) }     &  45.53(0.70)  & \multicolumn{1}{c|}{ 65.13(0.25)}     & 24.92(0.27)    \\ %\hline
FAT-Beta$^*$ & \multicolumn{1}{c|}{90.07(0.16) }     &   47.09(0.50)  & \multicolumn{1}{c|}{ 68.58(0.33) }     &  27.90(0.56)   & \multicolumn{1}{c|}{74.00(0.39)  }     &  45.12(0.90) & \multicolumn{1}{c|}{ 64.38(0.25)}     &  24.76(0.26)    \\ %\hline
FAT-Beta-EM$^*$   & \multicolumn{1}{c|}{89.86(0.06) }     &  48.61(0.13)   & \multicolumn{1}{c|}{67.95(0.24)}     &   28.06(0.24)    & \multicolumn{1}{c|}{ 74.78(0.10) }     &  45.75(0.48)     & \multicolumn{1}{c|}{ 64.32(0.21)}     &  23.57(0.14)   \\ \hline
TRADES      & \multicolumn{1}{c|}{ 87.31(0.27)}     &   53.07(0.23)   & \multicolumn{1}{c|}{62.83(0.33)  }     &  32.07(0.20)     & \multicolumn{1}{c|}{69.57(0.25)  }     &  47.07(0.37)  & \multicolumn{1}{c|}{ 58.16(0.38)}     &  27.82(0.23)   \\ %\hline
TRADES-EM$^*$   & \multicolumn{1}{c|}{  86.68(0.06)}     &  52.71(0.26)   & \multicolumn{1}{c|}{ 57.03(0.31) }     & 30.29(0.25)     & \multicolumn{1}{c|}{ 57.17(0.39)}     &  39.56(0.59)    & \multicolumn{1}{c|}{45.50(5.81)}     &   22.26(2.26)  \\ %\hline
TRADES-Beta$^*$ & \multicolumn{1}{c|}{ 89.81(0.22)}     &  47.50(0.78)   & \multicolumn{1}{c|}{62.61(0.36)  }     &  30.20(0.31)   & \multicolumn{1}{c|}{ 70.96(0.25)  }     & 46.74(0.23)   & \multicolumn{1}{c|}{ 57.72(0.24)}     &  23.49(0.21)   \\ %\hline
TRADES-Beta-EM$^*$   & \multicolumn{1}{c|}{86.99(0.10) }     &   51.85(0.23)   & \multicolumn{1}{c|}{62.13(0.34)}     &   30.52(0.20)  & \multicolumn{1}{c|}{69.44(0.25)}     &   46.24(0.39)    & \multicolumn{1}{c|}{ 56.03(0.15) }     &  22.90(0.32)  \\ \hline
\end{tabular}
}
\caption{Top-1 clean and robust accuracy comparison of AT baselines and the proposed AT-UR variants.}
\label{tab:top_1_acc}
\end{table}





\begin{table}[t]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{|c|cc|cc|cc|cc|}
\hline
     Dataset   & \multicolumn{2}{c|}{CIFAR10}     & \multicolumn{2}{c|}{CIFAR100}    & \multicolumn{2}{c|}{Caltech256}  & \multicolumn{2}{c|}{CUB200}      \\ \hline 
     Metric   & \multicolumn{1}{c|}{Cvg} & PSS & \multicolumn{1}{c|}{Cvg} & PSS & \multicolumn{1}{c|}{Cvg} & PSS & \multicolumn{1}{c|}{Cvg} & PSS \\ \hline
AT      & \multicolumn{1}{c|}{93.25(0.45)}     &   2.54(0.04)   & \multicolumn{1}{c|}{91.99 (0.61) }     &  14.29(0.59)    & \multicolumn{1}{c|}{94.35(0.81) }     &  23.73(1.68)   & \multicolumn{1}{c|}{91.87(0.90) }     &   17.75(0.71)  \\ %\hline
AT-EM$^*$   & \multicolumn{1}{c|}{92.36(0.53) }     &  \textbf{2.45(0.04)}    & \multicolumn{1}{c|}{91.87(0.61) }     & 13.29(0.49)     & \multicolumn{1}{c|}{93.41(0.58) }     &  21.19(1.46)    & \multicolumn{1}{c|}{91.26(0.57) }     &   \textbf{16.47(0.61)}  \\ %\hline
AT-Beta$^*$ & \multicolumn{1}{c|}{91.96(0.39)  }     &   2.50(0.04)   & \multicolumn{1}{c|}{ 91.24(0.69)  }     &  \textbf{11.61(0.40)}    & \multicolumn{1}{c|}{93.52(0.73) }     &   \textbf{18.54(1.32)}   & \multicolumn{1}{c|}{91.37(0.75)}     &   16.56(0.76)  \\ %\hline
AT-Beta-EM$^*$   & \multicolumn{1}{c|}{92.06(0.44)}     &  2.50(0.04)    & \multicolumn{1}{c|}{ 91.13(0.63) }     & 11.78(0.47)    & \multicolumn{1}{c|}{93.50(0.69)}     &   18.56(1.32)   & \multicolumn{1}{c|}{91.93(0.68)}     & 16.67(0.58)   \\ 
\hline
FAT      & \multicolumn{1}{c|}{93.007 (0.527)}     &   2.548 (0.048)   & \multicolumn{1}{c|}{92.043 (0.597)  }     &  13.596 (0.368)    & \multicolumn{1}{c|}{93.881 (0.451) }     &  22.848 (0.972)   & \multicolumn{1}{c|}{93.881 (0.451) }     &   22.848 (0.972) \\ %\hline
FAT-EM$^*$   & \multicolumn{1}{c|}{92.711 (0.657)  }     &  2.489 (0.049)    & \multicolumn{1}{c|}{91.634 (0.906) }     & 14.434 (2.121)    & \multicolumn{1}{c|}{93.520 (0.671)  }     &  21.811 (1.280)   & \multicolumn{1}{c|}{93.520 (0.671) }     &   \textbf{21.811 (1.280) }  \\ %\hline
FAT-Beta$^*$ & \multicolumn{1}{c|}{92.084 (0.544) }     &   2.547 (0.043)   & \multicolumn{1}{c|}{ 90.822 (0.489)  }     &  11.099 (0.255)    & \multicolumn{1}{c|}{93.495 (0.819) }     &   \textbf{18.070 (1.299)}   & \multicolumn{1}{c|}{93.495 (0.819)}     &   18.070 (1.299)  \\ %\hline
FAT-Beta-EM$^*$   & \multicolumn{1}{c|}{92.278 (0.296) }     &  2.433 (0.025)    & \multicolumn{1}{c|}{ 91.185 (0.551) }     & 11.087 (0.253)    & \multicolumn{1}{c|}{93.555 (0.563) }     &   18.161 (1.037)  & \multicolumn{1}{c|}{93.555 (0.563) }     & 18.161 (1.037)  \\ 
\hline
TRADES      & \multicolumn{1}{c|}{93.008 (0.456) }     &   2.492 (0.032)   & \multicolumn{1}{c|}{91.754 (0.720)  }     &  12.219 (0.498)   & \multicolumn{1}{c|}{94.328 (0.486)  }     &  22.820 (1.366)   & \multicolumn{1}{c|}{92.027 (0.586) }     &   22.294 (0.964) \\ %\hline
TRADES-EM$^*$   & \multicolumn{1}{c|}{92.225 (0.186)  }     &  2.330 (0.014)    & \multicolumn{1}{c|}{91.431 (0.766) }     & 12.386 (0.545)   & \multicolumn{1}{c|}{93.495 (0.651) }     &   15.027 (1.325)   & \multicolumn{1}{c|}{91.525 (0.818)}     &   17.797 (2.367)  \\ %\hline
TRADES-Beta$^*$ & \multicolumn{1}{c|}{92.431 (0.474) }     &   2.445 (0.040)  & \multicolumn{1}{c|}{ 91.196 (0.724) }     &  10.756 (0.436)    & \multicolumn{1}{c|}{93.547 (0.485)  }     &  17.016 (1.045)   & \multicolumn{1}{c|}{90.913 (0.894)}     &   18.191 (0.992) \\ %\hline
TRADES-Beta-EM$^*$   & \multicolumn{1}{c|}{92.117 (0.359)  }     &  2.419 (0.020)  & \multicolumn{1}{c|}{  91.219 (0.624) }     & 11.092 (0.382)    & \multicolumn{1}{c|}{93.128 (0.328) }     &   17.268 (0.724)  & \multicolumn{1}{c|}{90.956 (0.935)}     & 18.281 (1.224)   \\ 
\hline
\end{tabular}
}
\vspace{-0.3cm}
\caption{\textcolor{blue}{Comparison of AT and the proposed AT-UR variants denoted with $^*$ under AutoAttack \cite{croce2020reliable}. } }
\vspace{-0.5cm}
\label{tab:autoattack}
\end{table}



\section{ Proof of Theorem \ref{theorem:improved_generalization_bound_IW} }
\label{app_sec:proof_thm1}

\begin{theorem}
\label{theorem:appendix:improved_generalization_bound_IW}
(Theorem \ref{theorem:improved_generalization_bound_IW} restated, Beta weighting preserves generalization error bound.)
Suppose $\P_{(x, y) \sim \calP}\{ \hat r(x, y) = k \} = \frac{ k^{-c} }{ \sum_{k'=1}^K (k')^{-c}}$ is a polynomially decaying function with $c = \max\{ K^{-\alpha}, \frac{b \ln(a) + 1 }{ \ln(K) } + 2 - \alpha \}$ for $\alpha \geq 0$.
Beta weighting improves generalization error bound compared with ERM.
\end{theorem}


\begin{proof}
(of Theorem \ref{theorem:improved_generalization_bound_IW})

The key idea to prove Theorem \ref{theorem:improved_generalization_bound_IW} is to show $d_2(\calP || \calP / \omega) \leq d_2(\calP || \calP ) = 1$ (recall $d_2$ is the base-2 exponential for Ren\'yi divergence of order $2$, as in Lemma \ref{lemma:generalization_bound_iw}), which implies that Beta weighting gives tighter generalization error bound than ERM.

First, we derive the following equivalent formulations.
\begin{align*}
d_2(\calP || \calP / \omega)
= &
\int_{(x, y)} \calP(x, y) \cdot \omega(x, y) d(x, y)
=
\int_{(x, y)} \calP(x, y) \cdot p_\Beta(\hat r(x, y)/K; a, b) d(x, y)
\\
= &
\int_{(x, y)} \calP(x, y) \Bigg( \sum_{k=1}^K \I[\hat r(x, y) = 1] \Bigg) \cdot p_\Beta(\hat r(x, y)/K; a, b) d(x, y)
\\
= &
\sum_{k=1}^K \int_{(x, y)} \calP(x, y) \cdot \I[\hat r(x, y) = 1] \cdot p_\Beta(\hat r(x, y)/K; a, b) d(x, y)
\\
= &
\sum_{k=1}^K \int_{(x, y)} \calP(x, y) \cdot \I[\hat r(x, y) = 1] \cdot p_\Beta(k/K; a, b) d(x, y)
\\
= &
\sum_{k=1}^K \underbrace{ 
\P_{(x, y) \sim \calP}\{ \hat r(x, y) = k \} 
}_{ = p_k }
\cdot p_\Beta(k/K; a, b) .
\end{align*}

Suppose $p_k = \frac{ k^{-c} }{ \sum_{k'=1}^K (k')^{-c}}$ a polynomially decaying function of $k$ for $c \geq 0$.
\begin{align*}
&
p_k \cdot p_\Beta(k/K)
\\
= &
\frac{ k^{-c} }{ \sum_{k'=1}^K (k')^{-c} } \cdot \frac{ \Gamma(a+b) }{ \Gamma(a) \Gamma(b) } \cdot ( \frac{k}{K} )^{a-1} \cdot ( 1 - \frac{k}{K} )^{b-1}
\\
= &
\frac{ K^{-c} }{ K^{-c} } \cdot \frac{ k^{-c} }{ \sum_{k'=1}^K (k')^{-c} } \cdot \frac{ (a+b-1)! }{ (a-1)! (b-1)! } \cdot ( \frac{k}{K} )^{a-1} \cdot ( 1 - \frac{k}{K} )^{b-1}
\\
= &
\frac{ K^{-c} }{ \sum_{k'=1}^K (k')^{-c} } \cdot \frac{ k^{-c} }{ K^{-c} } \cdot \frac{ (a-c+b-1)! \cdot \prod_{i=a-c+b}^{a+b-1} i }{ (a-c-1)! (b-1)! \cdot \prod_{i=a-c}^{a-1} i } \cdot ( \frac{k}{K} )^{a-1} \cdot ( 1 - \frac{k}{K} )^{b-1}
\\
= &
\frac{ K^{-c} }{ \sum_{k'=1}^K (k')^{-c} } \cdot \frac{ \Gamma(a-c+b) }{ \Gamma(a-c) \Gamma(b) } \cdot \prod_{i=1}^c \frac{ a+b-c-1+i }{ a-c-1+i } \cdot ( \frac{k}{K} )^{a-c-1} \cdot ( 1 - \frac{k}{K} )^{b-1}
\\
= &
\underbrace{ 
\frac{ K^{-c} }{ \sum_{k'=1}^K (k')^{-c} }
}_{ = A}
\cdot 
\underbrace{ \prod_{i=1}^c ( 1 + \frac{ b }{ a-c-1+i } )
}_{ = B }\cdot 
\underbrace{
\frac{ \Gamma(a-c+b) }{ \Gamma(a-c) \Gamma(b) } \cdot ( \frac{k}{K} )^{a-c-1} \cdot ( 1 - \frac{k}{K} )^{b-1}
}_{ = p_\Beta(k/K; a-c, b) }
\end{align*}
where term $A$ can be bounded as follows
\begin{align*}
\frac{ K^{-c} }{ \sum_{k=1}^K k^{-c} }
\leq 
\frac{ K^{-c} ( c - 1 ) }{ 1 - ( K + 1 )^{-(c-1)} }
\leq 
c K^{-c}
% =
% \frac{ ( c - 1 ) ( K + 1 )^{c-1} }{ ( K + 1 )^{c-1} - 1 }
, ~~~ c > 0 ,
\end{align*}
and
term $B$ can be bounded as follows
\begin{align*}
B
= &
\prod_{i=1}^c ( 1 + \frac{b}{a-c-1+i} )
= 
\exp( \log( \prod_{i=1}^c ( 1 + \frac{b}{a-c-1+i} ) ))
\\
= &
\exp( \sum_{i=1}^c \log( 1 + \frac{b}{a-c-1+i} ) )
\leq 
\exp( \sum_{i=1}^c \frac{b}{a-c-1+i} )
\\
\leq &
\exp( \sum_{i=1}^{a-1} \frac{b}{i} )
\leq 
\exp( b ( \ln(a) + 1 ) ) .
\end{align*}



Then, combining term $A$ and $B$ together:
\begin{align*}
&~~
K^{-2} \cdot K^{-c+2} \cdot \exp( b \ln(a) + 1 ) \cdot c 
\leq 
K^{-2}
\\
\Leftrightarrow ~~&~~
\exp( \ln( K^{c-2} / c ) ) \geq \exp( b \ln(a) + 1 )
\\
\stackrel{(a)}{ \Leftarrow } ~~&~~
\exp( \ln( K^{c-2+\alpha} ) ) \geq \exp( b \ln(a) + 1 )
\\
\Leftrightarrow ~~&~~
c-2 + \alpha \geq \frac{b \ln(a) + 1 }{ \ln(K) }
\\
\Leftrightarrow ~~&~~
c \geq \frac{b \ln(a) + 1 }{ \ln(K) } + 2 - \alpha,
\end{align*}
where the development $(a)$ is due to $c = \max\{ K^{-\alpha}, \frac{b \ln(a) + 1 }{ \ln(K) } + 2 - \alpha \}$ for $\alpha \geq 0$.


As a result, we have 
\begin{align*}
&
p_k \cdot p_\Beta(k/K)
= 
K^{-2} \cdot p_\Beta(k/K; a-c; b)
\\
\Rightarrow &
\sum_{k=1}^K p_k \cdot p_\Beta(k/K; a-c; b)
\leq 
\sum_{k=1}^K p_\Beta(k/K; a-c; b) / K^2 
\leq
1 .
\end{align*}
% If $l \geq K / 3.5$, then for any $c > 0$, $\exp(-cl/K) \cdot \frac{ c - 1 }{ 1 - (K+1)^{-(c-1)} } \leq 1$.

% If $l \geq K / 2$, then for any $c > 0$, $\exp(-cl/K) \cdot \frac{ c - 1 }{ 1 - (K+1)^{-(c-1)} } \leq 1/2$.

% If $l \geq K / 1.5$, then for any $c > 0$, $\exp(-cl/K) \cdot \frac{ c - 1 }{ 1 - (K+1)^{-(c-1)} } \leq 0.3x$.

% Combining (\ref{eq:ub_prod_over_K}) and (\ref{eq:ub_inverse_poly_sum}), we have the first term done.
% This indicates that the generalization error bound can be improved by a factor of $\sqrt{\exp( - cl / K) \cdot \frac{a-1}{ 1 - (K+1)^{-(a-1)} } }$.

% If $cl=K$, then $\sqrt{ \exp(-1) } = 0.6065$.

% If $cl=0.75 K$, then $\sqrt{ \exp(-1) } = 0.6873$.

% If $cl=0.5 K$, then $\sqrt{ \exp(-1) } = 0.7788$.



% If $K=100, a=1.5$, then $\sqrt{ \frac{a-1}{ 1 - (K+1)^{-(a-1)} } } = 0.7452$.

% If $K=100, a=1.45$, then $\sqrt{ \frac{a-1}{ 1 - (K+1)^{-(a-1)} } } = 0.7173$.

% If $K=100, a=1.4$, then $\sqrt{ \frac{a-1}{ 1 - (K+1)^{-(a-1)} } } = 0.6892$.

% If $K=100, a=1.35$, then $\sqrt{ \frac{a-1}{ 1 - (K+1)^{-(a-1)} } } = 0.6610$.

% If $K=100, a=1.3$, then $\sqrt{ \frac{a-1}{ 1 - (K+1)^{-(a-1)} } } = 0.6326$.

% If $K=100, a=1.25$, then $\sqrt{ \frac{a-1}{ 1 - (K+1)^{-(a-1)} } } = 0.6043$.

% If $K=100, a=1.2$, then $\sqrt{ \frac{a-1}{ 1 - (K+1)^{-(a-1)} } } = 0.5761$.

% If $K=100, a=1.15$, then $\sqrt{ \frac{a-1}{ 1 - (K+1)^{-(a-1)} } } = 0.5480$.

% If $K=100, a=1.1$, then $\sqrt{ \frac{a-1}{ 1 - (K+1)^{-(a-1)} } } = 0.5201$.

% If $K=100, a=1.05$, then $\sqrt{ \frac{a-1}{ 1 - (K+1)^{-(a-1)} } } = 0.4926$.

% If $K=100, a=1.01$, then $\sqrt{ \frac{a-1}{ 1 - (K+1)^{-(a-1)} } } = 0.4709$.




% If $K=10, a=1.5$, then $\sqrt{ \frac{a-1}{ 1 - (K+1)^{-(a-1)} } } = 0.8461$.

% If $K=10, a=1.4$, then $\sqrt{ \frac{a-1}{ 1 - (K+1)^{-(a-1)} } } = 0.8053$.

% If $K=10, a=1.3$, then $\sqrt{ \frac{a-1}{ 1 - (K+1)^{-(a-1)} } } = 0.7648$.

% If $K=10, a=1.2$, then $\sqrt{ \frac{a-1}{ 1 - (K+1)^{-(a-1)} } } = 0.7246$.

% If $K=10, a=1.1$, then $\sqrt{ \frac{a-1}{ 1 - (K+1)^{-(a-1)} } } = 0.6849$.

% If $K=10, a=1.05$, then $\sqrt{ \frac{a-1}{ 1 - (K+1)^{-(a-1)} } } = 0.6652$.

% If $K=10, a=1.01$, then $\sqrt{ \frac{a-1}{ 1 - (K+1)^{-(a-1)} } } = 0.6497$.


% Case 2: suppose $p_k = \frac{ \exp( - \frac{ k^2 }{ \sigma^2 } ) }{ \sum_{k'=1}^K \exp( - \frac{ k^2 }{ \sigma^2 } ) }$ a sub-Gaussian-shape function of $k$ for $c \geq 0$.
% \begin{align*}
% &
% p_k \cdot p_\Beta(k/K)
% \\
% = &
% \frac{ \exp( - \frac{ k^2 }{ \sigma^2 } ) }{ \sum_{k'=1}^K \exp( - \frac{ k^2 }{ \sigma^2 } ) } \cdot \frac{ \Gamma(a+b) }{ \Gamma(a) \Gamma(b) } \cdot ( \frac{k}{K} )^{c-1} \cdot ( 1 - \frac{k}{K} )^{b-1}
% \end{align*}



% Case 3: suppose $p_k = \frac{ \exp( - \frac{ k }{ \sigma } ) }{ \sum_{k'=1}^K \exp( - \frac{ k }{ \sigma } ) }$ a sub-Exponential-shape function of $k$ for $c \geq 0$.
% \begin{align*}
% &
% p_k \cdot p_\Beta(k/K)
% \\
% = &
% \frac{ \exp( - \frac{ k }{ \sigma } ) }{ \sum_{k'=1}^K \exp( - \frac{ k }{ \sigma } ) } \cdot \frac{ \Gamma(a+b) }{ \Gamma(a) \Gamma(b) } \cdot ( \frac{k}{K} )^{c-1} \cdot ( 1 - \frac{k}{K} )^{b-1}
% \end{align*}
\end{proof}

\yanblue{
(1)
\begin{align*}
\sum_{k=1}^K k^{-c}
\geq 
\int_{1}^{K+1} k^{-c} dk
=
\frac{ k^{-(c-1)} }{ -(c-1) } \bigg|_{k=1}^{K+1}
=
\frac{ (K+1)^{-(c-1)} }{ -(c-1) } - \frac{ 1^{-(c-1)} }{ -(c-1) }
=
\frac{ (K+1)^{-(c-1)} - 1 }{ - (c-1) } ,
\end{align*}
where the inequality is due to the left Riemann sum for the monotonically decreasing function $k^{-c}$ with $c > 0$.
}
% \begin{lemma}
% \label{lemma:partial_sum_of_series}
% (Partial sum of some series)
% \begin{align*}
% 1) 
% &
% \sum_{k=1}^K k^a
% \leq 
% \frac{ (K+1)^{a+1} }{ a + 1 }
% \\
% 2)
% &
% \ln(K)
% \leq 
% \sum_{k=1}^K \frac{1}{k}
% \leq 
% \ln(K) + 1,
% \\
% \yanred{
% 3)}
% &
% \sum_{k=1}^K k^{-a} 
% \leq 
% \frac{1}{a-1}, \text{ for } a > 1.
% \end{align*}
% \end{lemma}

% \begin{proof}
% (of Lemma \ref{lemma:partial_sum_of_series})

% $3)$
% For $a > 1$:
% \begin{align*}
% \sum_{k=1}^K k^{-a}
% \leq 
% \int_{0}^{K} k^{-a}
% =
% - \frac{ K^{-(a-1)} }{ a - 1 } + \frac{ 0^{-(a-1)} }{ a - 1 } 
% =
% \frac{ 1 - 1 / K^{ a - 1 } }{ a - 1 }
% \leq 
% \frac{ 1 }{ a - 1 } .
% \end{align*}

% \begin{align*}
% \sum_{k=1}^K k^{-a}
% \geq 
% \int_{1}^{K+1} k^{-a} dk
% =
% \frac{ k^{-a+1} }{ -a + 1 } \bigg|_{1}^{K+1}
% =
% \frac{ (K+1)^{-a+1} }{ -a + 1 } - \frac{ 1^{-a+1} }{ -a + 1 } 
% =
% \frac{ 1 - (K+1)^{-a+1} }{ a - 1 }
% \end{align*}


% When $1.01 \leq a \leq 1.2$ and $K \geq 10$, the above lower bound can be specified as
% \begin{align*}
% \sum_{k=1}^K k^{-a}
% \geq 
% \frac{ 1 - ( K + 1 )^{ -a + 1 } }{ a - 1 }
% \geq 
% 1 - 11^{-a+1}
% \geq 
% 0.2 .
% \end{align*}


% $4)$: when rank is distributed by sub-Gaussian and mean of $p_\Beta$ is around $\bar k$.

% Case 1, for $k \leq \bar k$:
% \begin{align*}
% &
% \sum_{k=1}^{\bar k} \exp( - k^2) \cdot \exp( - (\bar k - k )^2 )
% = 
% \sum_{k=1}^{\bar k} \exp( - k^2 - k^2 - \bar k^2 + 2 \bar k k )
% \\
% = &
% \sum_{k=1}^{\bar k} \exp( - 2 k^2 - \bar k^2 + 2 \bar k k )
% =
% \sum_{k=1}^{\bar k} \exp( - 2 k ( k - \bar k ) - \bar k^2 )
% \stackrel{ (a) }{ \leq }
% \sum_{k=1}^{\bar k} \exp( \bar k^2 / 2 - \bar k^2 )
% \\
% = &
% \sum_{k=1}^{\bar k} \exp( - \bar k^2 / 2 )
% =
% \bar k \exp( - \bar k^2 / 2 ) ,
% \end{align*}
% where the inequality $(a)$ is due to $-2k(k-\bar k) \leq \bar k^2 / 2$.
% If $\bar k = 1$, $\bar k \exp(-\bar k^2 / 2)=0.6065$.
% If $\bar k = 2$, $\bar k \exp(-\bar k^2 / 2)=0.2707$.
% If $\bar k = 3$, $\bar k \exp(-\bar k^2 / 2)=0.0333$.
% If $\bar k = 4$, $\bar k \exp(-\bar k^2 / 2)=0.0013$.
% If $\bar k = 5$, $\bar k \exp(-\bar k^2 / 2)=0.000018633$.

% Case 2, for $k > \bar k$:
% \begin{align*}
% &
% \sum_{k = \bar k+1}^K \exp( - k^2 ) \cdot \exp(-( \bar k - k )^2)
% \leq 
% \sum_{k=\bar k+1}^{K} \exp( - k^2 ) \cdot k
% \leq 
% \int_{ \bar k }^{ K } \exp( - k^2 ) \cdot k dk
% \\
% = &
% - \exp(-(K+1)^2) / 2 + \exp(-(\bar k)^2) / 2 
% \leq 
% \exp(-\bar k^2) / 2
% \leq 
% \exp( -9 ) / 2
% =
% 0.0111 .
% \end{align*}
% As a result, combining two cases gives improved generalization bound ($<1$, which is in the ERM case).


% $5)$ When rank is distributed by sub-exponential and mean of $p_\Beta$ is around $\bar k$.

% Case 1, for $k \leq \bar k$:
% \begin{align*}
% & 
% \sum_{k=1}^{\bar k} \exp( - k ) \cdot \exp( - ( \bar k - k )^2 )
% =
% \sum_{k=1}^{\bar k} \exp( - k - ( \bar k - k )^2 )
% =
% \sum_{k=1}^{\bar k} \exp( - \bar k^2 - k ( k + 1 - 2 \bar k ) )
% \\
% \leq &
% \sum_{k=1}^{\bar k} \exp( - \bar k^2 + \frac{1-2\bar k}{2} ( - \frac{1-2\bar k}{2} + 1 - 2 \bar k ) )
% =
% \sum_{k=1}^{\bar k} \exp( - \bar k^2 + ( \frac{1-2\bar k}{2} )^2 )
% \\
% = &
% \sum_{k=1}^{\bar k} \exp( - \bar k^2 + \bar k^2 - \bar k + 1 / 4)
% =
% \sum_{k=1}^{\bar k} \exp( - \bar k + 1 / 4)
% =
% \bar k \exp( - \bar k + 1 / 4),
% \end{align*}
% where the inequality is due to $- k (k+1-2 \bar k) \leq - \frac{1-2 \bar k}{2} (-\frac{1-2 \bar k}{2}+1-2 \bar k)$.
% If $\bar k = 1$, $\bar k \exp(-\bar k - 1/4)=0.4724$.
% If $\bar k = 2$, $\bar k \exp(-\bar k - 1/4)=0.3475$.
% If $\bar k = 3$, $\bar k \exp(-\bar k - 1/4)=0.1918$.
% If $\bar k = 4$, $\bar k \exp(-\bar k - 1/4)=0.0941$.
% If $\bar k = 5$, $\bar k \exp(-\bar k - 1/4)=0.0433$.
% If $\bar k = 6$, $\bar k \exp(-\bar k - 1/4)=0.0191$.
% If $\bar k = 7$, $\bar k \exp(-\bar k - 1/4)=0.0082$.
% If $\bar k = 8$, $\bar k \exp(-\bar k - 1/4)=0.0034$.
% If $\bar k = 9$, $\bar k \exp(-\bar k - 1/4)=0.0014$.
% If $\bar k = 10$, $\bar k \exp(-\bar k - 1/4)=0.00058295$.




% Case 2, for $k > \bar k$:
% \begin{align*}
% &
% \sum_{k=\bar k+1}^{K} \exp( - k ) \cdot \exp( - ( \bar k - k )^2 )
% \leq 
% \sum_{k=\bar k+1}^{K} \exp( - k ) \cdot \exp( - 1 )
% \leq 
% \int_{\bar k}^K \exp( - k ) dk \cdot \exp( - 1 )
% \\
% = &
% ( - \exp(-K) + \exp(-\bar k) ) \cdot \exp( - 1 )
% \leq 
% \exp( - 1 ) \cdot \exp( - 1 )
% =
% \exp(-2)
% =
% 0.1353 ,
% \end{align*}
% where the last inequality is due to $\bar k \geq 1$.


% $5)$ when rank is distributed by polynomial with degree $-a < -1$ and mean of $p_\Beta$ is around $\bar k$.


% Case 1, for $k \leq \bar k$:
% \begin{align*}
% & 
% \sum_{k=1}^{\bar k} k^{-a} \cdot \exp( - ( \bar k - k )^2 )
% =
% \sum_{k=2}^{\bar k-1} k^{-a} \cdot \exp( - ( \bar k - k )^2 )
% + 1^{-a} \cdot \exp(-( \bar  k - 1 )^2)
% + \bar k^{-a} \cdot 1
% \\
% = &
% \end{align*}


% Case 2, for $k \geq \bar k + 1$:
% \begin{align*}
% & 
% \sum_{k=\bar k+1}^{K} k^{-a} \cdot \exp( - ( \bar k - k )^2 )
% \end{align*}
% \end{proof}



% \CUT{
% \begin{theorem}
% \label{theorem:improved_PS_IW}
% (IW reduces expected prediction set sizes in CP.)
% \end{theorem}
% \NOTE{Do we need this theorem?}

% \begin{proof}
% (of Theorem \ref{theorem:improved_PS_IW})

% \begin{align*}
% \E_X[ | \calC(X) | ]
% \leq 
% \sum_{k=1}^K k \cdot \frac{ p_\Beta(k/K; a-c, b) }{ K }
% \leq 
% \sum_{k=1}^K B(a, b) \cdot (\frac{k}{K})^{a-c} \cdot (1-\frac{k}{K})^{b-1}
% \end{align*}
% \end{proof}
% }





\begin{align*}
\Gamma(z)
=
\int_0^\infty t^{z-1} \exp(-t) dt
=
\frac{1}{z \exp(\gamma z)} \prod_{i=1}^\infty (1+\frac{z}{i}) \exp(-\frac{z}{i}) ,
\end{align*}
where the second equality is due to Weierstrass's definition for Gamma function.



\begin{align*}
\frac{ \Gamma(a+b) }{ \Gamma(a) \Gamma(b) }
=
\frac{ \Gamma(a+b+c) }{ \Gamma(a) \Gamma(b+c) } \cdot 
\underbrace{ \frac{\Gamma(a+b) \Gamma(b+c)}{\Gamma(a+b+c) \Gamma(b)} }_{ = A }
\end{align*}


\begin{align*}
A 
= &
\frac{\Gamma(a+b) \Gamma(b+c)}{\Gamma(a+b+c) \Gamma(b)}
\\
= &
\frac{ (a+b+c) \exp(\gamma (a+b+c)) b \exp(\gamma(b)) }{ (a+b) \exp(\gamma (a+b)) (b+c) \exp(\gamma(b+c)) } 
\prod_{i=1}^\infty \frac{ (1+\frac{a+b}{i}) (1+\frac{b+c}{i}) }{ (1+\frac{a+b+c}{i}) (1+\frac{b}{i}) } \exp( - \frac{ 0 }{ i } )
\\
= &
\underbrace{ 
\frac{ b(a+b+c) }{(a+b)(b+c)}
}_{ \leq 1 }
\underbrace{ 
\prod_{i=1}^\infty \frac{ (i+a+b) (i+b+c) }{ (i+a+b+c) (i+b) }
}_{ = B }
\end{align*}


\begin{align*}
B 
= &
\prod_{i=1}^\infty \frac{ (i+a+b) (i+b+c) }{ (i+a+b+c) (i+b) }
=
\exp( \sum_{i=1}^\infty \ln( \frac{ (i+a+b) (i+b+c) }{ (i+a+b+c) (i+b) } ) )
\\
= &
\exp( \sum_{i=1}^\infty \ln( (1+\frac{a}{i+b}) (1-\frac{a}{i+a+b+c}) ) )
\\
= &
\exp( \sum_{i=1}^\infty \ln( 1 + \frac{ac}{(i+b)(i+a+b+c)} ) )
\\
\leq &
\exp( \sum_{i=1}^\infty \ln( 1 + \frac{ac}{i^2} ) )
\leq 
\exp( \ln( \frac{1}{1-\sqrt{ac}} ) )
=
\frac{1}{1-\sqrt{ac}} ,
% \\
% \leq &
% \exp( \sum_{i=1}^\infty \ln( 1 + \frac{ac}{(i+b)(i+a+b+c)} ) )
\end{align*}
where the first inequality is due to $b, c \geq 0$, and the second inequality is due to partial sum below for $0 \leq ac < 1$.


Partial sum:
\begin{align*}
\sum_{i=1}^n \ln(1+\frac{a}{i^2})
= &
- \sum_{i=1}^n \ln(\frac{i^2}{i^2+a})
=
- \sum_{i=1}^n \ln(\frac{i^2}{i^2+a})
=
- \sum_{i=1}^n \ln( 1 - \frac{a}{i^2+a})
\\
\leq &
- \sum_{i=1}^n \ln( 1 - \frac{a}{i^2})
=
- \sum_{i=1}^n \ln( \frac{i^2 - a}{i^2})
=
- \sum_{i=1}^n \ln( \frac{ (i + \sqrt{a}) }{i} \cdot \frac{ (i-\sqrt{a}) }{i} )
\\
= &
- \sum_{i=1}^n \Bigg( \ln( \frac{ i + \sqrt{a} }{i} ) - \ln( \frac{i}{ i-\sqrt{a} } ) \Bigg)
=
- \sum_{i=1}^n \ln(\frac{i+\sqrt{a}}{i}) 
+ \sum_{i=1}^n \ln(\frac{i}{i-\sqrt{a}})
\\
= &
- \sum_{i=1}^{n-1} \ln(\frac{i+\sqrt{a}}{i}) 
- \ln(\frac{n+\sqrt{a}}{n}) 
+ \sum_{i=2}^n \ln(\frac{i}{i-\sqrt{a}})
+ \ln(\frac{1}{1-\sqrt{a}})
\\
= &
- \sum_{i=1}^{n-1} \ln(\frac{i+\sqrt{a}}{i}) 
+ \sum_{i=1}^{n-1} \ln(\frac{i+1}{i+1-\sqrt{a}})
- \ln(\frac{n+\sqrt{a}}{n}) 
+ \ln(\frac{1}{1-\sqrt{a}})
\\
\leq &
\ln(\frac{1}{1-\sqrt{a}}) ,
\end{align*}
where the first inequality is due to $0 \leq a$ and the last inequality is due to $a < 1$.



\begin{align*}
&
p_k \cdot p_\Beta(k/K; a, b)
\\
= &
\frac{ k^{-c} }{ \sum_{k'=1}^K (k')^{-c} } \cdot \frac{ \Gamma(a+b) }{ \Gamma(a) \Gamma(b) } \cdot ( \frac{k}{K} )^{a-1} \cdot ( 1 - \frac{k}{K} )^{b-1}
\\
\leq &
\frac{ k^{-c} }{ \sum_{k'=1}^K (k')^{-c} } \cdot \frac{ \Gamma(a+b+c) }{ \Gamma(a) \Gamma(b+c) } \cdot \frac{1}{1-\sqrt{ac}} \cdot 
(\frac{k}{K})^{a-1} (1-\frac{k}{K})^{b+c-1} \cdot (1-\frac{k}{K})^{-c}
\\
= &
\underbrace{
k^{-c} \cdot \frac{ c-1 }{ 1 - (K+1)^{-c+1} } \cdot \frac{1}{1-\sqrt{ac}} \cdot (1-\frac{k}{K})^{-c}
}_{ = \widehat p_k}
\cdot p_\Beta(k/K; a, b+c)
\end{align*}

\yanred{Still missing: $\sum_{k=1}^K \widehat p_k \cdot p_\Beta(k/K; a, b+c)\leq O(1)$? This upper bound may exceed $1$, but should be still OK if can be a constant such as $30$, since it does not increase the growth rate of the generalization error bound under ERM.}




For cost-sensitive-type weighting in Beta distribution:
\begin{align*}
&
( 1 - \lambda ) R(f) + \lambda \rank(f)
\\
= &
( 1 - \lambda ) \sum_{k=1}^K \P\{ r_f(x, y) = k \} \cdot \E[ \I[ h(x) \neq y ] | r_f(x, y) = k ] + \lambda \rank(f)
\\
&
+ \lambda \sum_{k=1}^K \P\{ r_f(x, y) = k \} \cdot k
\\
= &
\sum_{k=1}^K \P\{ r_f(x, y) = k \} \cdot ( (1-\lambda) \E[ \I[ h(x) \neq y ] | r_f(x, y) = k ] + \lambda k )
\\
\leq &
\sum_{k=1}^K \P\{ r_f(x, y) = k \} \cdot ( (1-\lambda) \E[ \ell(f(x), y)) | r_f(x, y) = k ] + \lambda k )
\\
\leq &
\sum_{k=1}^K \P\{ r_f(x, y) = k \} \cdot ( (1-\lambda) \E[ \ell(f(x), y)) | r_f(x, y) = k ] + \lambda \sigma_k \E[ \ell(f(x), y) | r_f(x, y) = k ] )
\\
= &
\sum_{k=1}^K 
\underbrace{
\P\{ r_f(x, y) = k \}
}_{ = p_k^\exponential }
\cdot \Big( (1 - \lambda + \lambda \sigma_k) \E\big[ \ell(f(x), y) \big| r_f(x, y) = k \big] \Big)
,
\end{align*}
where the first inequality is due to surrogate loss,
the second inequality is due to the assumption $k \leq \sigma_k \cdot \E[ \ell(f(x), y) | r_f(x, y) = k ]$.

\yanred{Missing: we can simply focus only on $\lambda \sigma_k$ part, instead of the overall weights, right?}

Task: show $\{ \frac{ p_k \cdot k }{ - \log(f(x)_k) } \}_{k=1}^K$ are Beta-like.
Assume: $p_k = \frac{ \exp(-k) }{ \sum_{k'=1}^K \exp(-k') }$, and
$f(x)_k \leq M - (k/K)^a$.

Now we start:
\begin{align*}
\frac{ p_k \cdot k }{ - \log(f(x)_k) }
\leq 
\frac{ \exp(-k) \cdot k  }{ - ( f(x)_k - 1 ) }
\leq 
\frac{ \exp( -k + \ln(k) ) }{ 1 - M + (k/K)^\beta }
\leq 
\Bigg( \frac{K-k}{K} \Bigg)^b
\cdot \frac{ K }{ 1 - M } \cdot \bigg( \frac{ k }{ K } \bigg)^a
,
\end{align*}
where the first inequality is due to $1+\ln(x) \leq x$,
the second inequality is due to two lemmas.


Lemma:
\begin{align*}
\Bigg( \frac{K}{K-k} \Bigg)^b
\leq 
\exp(k - \ln(k))
\end{align*}

Lemma:
\begin{align*}
\frac{1}{b+c} 
\leq 
\frac{ d c }{b}
\Leftrightarrow 
b 
\leq 
\frac{d c^2}{1-dc}
\end{align*}

Lemma:
\begin{align*}
1 - M 
\leq 
\frac{ K (k/K)^{2a} }{ 1 - K (k/K)^{a} }
\end{align*}

\yanred{Still missing: lower bound with Beta PDF?}


\yanred{Still missing: $p_k$ can be exp or poly, so generalization and cost-sensitive analysis should be consistent (now they are not)}

